Pricing for Information Revelation in Demand Response: A Strategic Communication Approach

Demand response aggregators require consumers' private flexibility information to dispatch loads efficiently. Yet self-interested consumers have incentives to misreport it. This paper investigates how much information heterogeneous consumers can credibly convey through nonbinding, unverifiable reports, and how a pre-announced retail tariff can improve this revelation. We model this interaction as a multi-sender strategic communication game with state-dependent bias, using the cheap-talk framework. The aggregator maximizes social welfare, and consumers have private valuations and quadratic payoffs. Closed-form conditions identify when the set of dispatched consumers is invariant to the reports. Under these conditions, reporting incentives decouple into independent single-sender subgames. We derive a closed-form uniform tariff that simultaneously minimizes the mean-squared strategic bias of all dispatched consumers. In this regime, the welfare loss relative to full communication is expressed as a weighted sum of residual posterior variances, showing that every equilibrium weakly improves expected social welfare over no communication. Numerical studies support the theoretical results and show that, when consumers coordinate on informative equilibria, strategic communication with the proposed bias-minimizing tariff recovers most of the full-communication welfare gain over no communication.

==> latexmkrc <==
add_cus_dep('tex', 'aux', 0, 'makeexternaldocument');

sub makeexternaldocument {
    if (!($root_filename eq $_[0])) {
        system("latexmk -cd -pdf \"$_[0]\"");
    }
}

